Beyond Isolated Tasks: A Framework for Evaluating Coding Agents on Sequential Software Evolution

Existing datasets for coding agents evaluate performance on isolated, single pull request (PR) tasks in a stateless manner, failing to capture the reality of real-world software development where code changes accumulate, technical debt accrues, and test suites grow over time. To bridge this gap, we introduce an automated coding task generation framework, which helps generate our dataset SWE-STEPS, that evaluates coding agents on long-horizon tasks through two realistic settings mirroring actual developer workflows: Conversational coding with iterative requests, and single-shot Project Requirement document (PRD)-based coding. Unlike existing datasets that evaluate agents on disjointed Pull Requests (PRs), our framework assesses performance across chains of dependent PRs, enabling evaluation of sequential execution, regression verification, and long-term repository health. We discover that widely used isolated PR evaluations yield inflated success rates, w.r.t. our settings - overshooting performance by as much as 20 percentage points - because they ignore the ``spillover'' effects of previous inefficient or buggy code. Furthermore, our analysis reveals that even when agents successfully resolve issues, they degrade repository health by generating code with higher cognitive complexity and technical debt compared to human developers, underscoring the necessity for multidimensional evaluation.

==> Figures/error_analysis_trace.tex <==
% --- START FIGURE SNIPPET ---
% \begin{figure}[t] % 't' attempts to place it at the top of the page
%     \centering
%     \small
%     % Outer container
%     \begin{tcolorbox}[
%         title={\textbf{Agent Failure: Solving Previous Issues}},
%         colback=white,
%         colframe=gray!50!black,
%         boxrule=0.8pt,
%         arc=3pt
%     ]
%         % 1. The Prompt
%         \textbf{Input Prompt (PR \#62848):} Fix bug in \texttt{pd.json\_normalize} where \texttt{max\_level} raises \texttt{AttributeError} on non-dict items.
        
%         \vspace{4pt} \hrule \vspace{4pt}

%         % 2. The Execution
%         \textbf{Execution Trace:}
%         \begin{itemize} \setlength\itemsep{0em}
%             \item \textbf{Step 1 (Correct):} Agent writes a fix for \texttt{json\_normalize}.
%             \item \textbf{Step 2 (Observation):} Agent runs tests. The logs display results for \texttt{test\_aggregate.py} (related to the \textit{previous}, already completed PR \#62729).
%         \end{itemize}

%         % 3. The Error (Highlighting the thought process)
%         \begin{tcolorbox}[colback=yellow!10, colframe=yellow!60!black, title=Agent Thought Process, left=2pt, right=2pt, top=1pt, bottom=1pt]
%             "Since I see tests for PR \#62729 appearing in the summary, I must have missed something there. I will rewrite the \texttt{NamedAgg} functionality to ensure it accepts \texttt{*args} and \texttt{**kwargs}."
%         \end{tcolorbox}

%         % 4. The Result
%         \begin{itemize} \setlength\itemsep{0em}
%             \item \textbf{Step 3 (Deviation):} Agent reverts work on PR \#62848 and starts re-implementing PR \#62729.
%             \item \textbf{Outcome:} \textcolor{red}{\textbf{FAILED}}. The agent exhausts its budget solving a previous PR that has already been solved.
%         \end{itemize}
%     \end{tcolorbox}
%     \caption{An example of \textit{Goal Drift}. The agent conflates the current task (PR 62848) with artifacts found in the environment from a previous task (PR 62729), leading to task abandonment. }
%     \label{fig:failure_trace}
% \end{figure}
% --- END FIGURE SNIPPET ---

\begin{figure}[t]
    \centering
    % Define specific colors for this chart locally to avoid conflicts
    \definecolor{bg_gray}{RGB}{245, 245, 245}
    \definecolor{bg_yellow}{RGB}{255, 252, 235}
    \definecolor{border_gray}{RGB}{100, 100, 100}

    \begin{tcolorbox}[
        colback=white,
        colframe=border_gray,
        title={\textbf{Failure Mode: Solving Previous Issues}},
        fonttitle=\bfseries,
        boxrule=1pt,
        arc=2pt,
        width=\linewidth
    ]
        % --- 1. TASK DEFINITION ---
        \textbf{\small Task Assignment (Pandas - PR \#62848)} \par
        \footnotesize
        Fix a bug in \texttt{pd.json\_normalize} where an \texttt{AttributeError} was raised if \texttt{max\_level} was set to an integer and input data contained non-dict items.
        
        \vspace{0.2cm}
        \hrule
        \vspace{0.2cm}

        % --- 2. THE TRIGGER (OBSERVATION) ---
        \textbf{\small Cycle 1: Observation } \par
         The agent tries to solve the given task. The agent runs tests. The environment (shared with previous tasks) displays residual logs from a \textit{different} PR (\#62729).
        \vspace{2pt}
        \begin{tcolorbox}[
            colback=bg_gray, 
            boxrule=0pt, 
            frame hidden, 
            left=2pt, right=2pt, top=2pt, bottom=2pt
        ]
            \tiny \ttfamily
            pytest pandas/tests/groupby/aggregate/test\_aggregate.py \\
            ... \\
            PASSED pandas/tests/groupby/aggregate/test\_aggregate.py \\
            (Test case summary: All tests passed for NamedAgg support)
        \end{tcolorbox}
        \vspace{0.2cm}

        % --- 3. THE ERROR (THOUGHT PROCESS) ---
        \textbf{\small Cycle 2: Reflection } \par
        The agent hallucinates that the passed tests for the \textit{previous} PR are actually the requirements for the \textit{current} PR.
        \vspace{2pt}
        \begin{tcolorbox}[
            colback=bg_yellow, 
            colframe=orange!50!yellow, 
            boxrule=0.5pt,
            left=2pt, right=2pt, top=2pt, bottom=2pt
        ]
            \textit{"I see the tests for \texttt{test\_aggregate.py} are passing. Wait, looking at the logs, it seems I am interacting with the \texttt{NamedAgg} functionality (PR \#62729). I will rewrite the functionality to match PR \#62729."}
        \end{tcolorbox}

        \vspace{0.2cm}
        \hrule
        \vspace{0.2cm}

        % --- 4. OUTCOME ---
        \textbf{\small Outcome} \par
        \textbf{Failure.} The agent implemented support for \texttt{NamedAgg} (PR \#62729) instead of fixing \texttt{json\_normalize} (PR \#62848). The original issue remains unresolved.

    \end{tcolorbox}
    \caption{An example of \textit{Goal Drift}. The agent conflates the current task (PR \#62848) with artifacts found in the environment from a previous task (PR \#62729), leading to task abandonment. }
    \label{fig:goal_drift_trace}
\end{figure}

==> Figures/fig_co_relation_analysis.tex <==
% \begin{figure}[h]
%     \centering
%     \includegraphics[width=0.9\textwidth]{co_relation_analysis_graphs.png}
%     \caption{Your caption here}
%     \label{fig:corelation_analysis}
% \end{figure}

\begin{figure*}[t]
    \centering
    \includegraphics[width=0.9\textwidth]{Figures/co_relation_analysis_graphs.png}
    \caption{Comparison of results across six different experimental conditions. (Top row) Conditions A, B, and C. (Bottom row) Conditions D, E, and F.}
    \label{fig:corelation_analysis}
\end{figure*}

==> Figures/fig_task_split.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=0.8\textwidth]{Figures/tasks_split.png}
    \caption{Composition of all the versions of the dataset - Total, Lite and Mini, difficulty-wise}
    \label{fig:corelation_analysis}
\end{figure*}

==> Figures/figure_agent_eval_setting.tex <==
% --- FIGURE 2 & 3: Agent Workflows (Side-by-Side) ---
\begin{figure*}[t]
    \centering
    % -- LEFT SIDE: Image 2 --
    \begin{subfigure}[b]{0.48\textwidth}
        \centering
        % Replace with your actual filename for Image 2
        \includegraphics[width=\linewidth]{Figures/global_setting.pdf}
        \caption{Basic Agent Loop}
        \label{fig:agent_global}
    \end{subfigure}
    \hfill % Adds space between the two images
    % -- RIGHT SIDE: Image 3 --
    \begin{subfigure}[b]{0.48\textwidth}
        \centering
        % Replace with your actual filename for Image 3
        \includegraphics[width=\linewidth]{Figures/prd_setting.pdf}
        \caption{PRD-Enhanced Agent Loop}
        \label{fig:agent_prd}
    \end{subfigure}
    
    % Main caption for the group
    \caption{\textbf{Comparison of Agent Workflows.} (a) The standard agent directly implements fixes based on feedback. (b) The enhanced agent generates a PRD document first to plan the implementation.}
    \label{fig:agent_setting_comparison}
\end{figure*}

==> Figures/figure_data_extraction.tex <==

% --- FIGURE 1: Task Extraction (Single Column) ---
\begin{figure}[t]
    \centering
    % Replace with your actual filename for Image 1
    \includegraphics[width=\linewidth]{Figures/task_generation_diagram.pdf}
    \caption{\textbf{Task Extraction Pipeline.} 
    Tasks are extracted from PRs and verified via the execution sandbox.}
    \label{fig:task_extraction}
\end{figure}

==> Figures/figure_perf_vs_chain_and_perf_vs_tests.tex <==
\begin{figure*}[t]
        % --- Single Common Caption ---
 \caption{\textbf{Pass Rate Analysis.} 
Comparison of Average PR Pass Rates for Claude, Gemini, and GPT models relative to the total number of PRs (top) and test suite size (bottom). 
The plots reveal that the \textit{Individual PR} setting consistently maintains higher pass rates compared to \textit{Global Memory} and \textit{PRD} strategies, particularly as the complexity and number of tests increase.}
\label{fig:pass_rate_analysis}
    \centering
    
    % --- Top Image ---
    \includegraphics[width=\textwidth]{Figures/perf_vs_chain.png} 
    
    % Force a line break and add vertical space between the images
    \par\vspace{0.5cm}
    
    % --- Bottom Image ---
    \includegraphics[width=\textwidth]{Figures/perf_vs_test.png}
    
\end{figure*}

==> Figures/figure_sonarqube.tex <==
\begin{figure*}[t]
    \centering
    
    % --- CAPTION MOVED TO TOP ---
    \caption{\textbf{Comparative Analysis of Code Quality Evolution.} 
    The figure illustrates the progression of $\Delta$ Cognitive Complexity (top row) and $\Delta$ SQALE Index (bottom row) across three experimental repositories: \texttt{conan}, \texttt{haystack}, and \texttt{moto}. 
    Performance is evaluated across five difficulty bins (Bin 1--5) for three Large Language Model agents (Gemini 3.0 Pro, Claude Sonnet 4.5, GPT 5.2 Chat) versus the human ground truth (\textit{Gold Trace}). 
    The plots reveal that while the Gold Trace maintains a near-zero or low fluctuation in complexity and technical debt, the autonomous agents tend to introduce significantly higher complexity and debt accumulation, particularly in higher bins.}
    \label{fig:six_grid_complexity}
    
    % Optional: Add a small space so the images don't touch the caption text
    \vspace{0.2cm} 
    
    % --- ROW 1 ---
    % 0.33\textwidth ensures they take up 33% of the page width each (tight fit)
    \begin{subfigure}{0.33\textwidth}
        \centering
        \includegraphics[width=\linewidth]{Figures/cognitive_complexity_conan.png}
    \end{subfigure}% <--- The % is required to prevent a white space gap
    \hfill
    \begin{subfigure}{0.33\textwidth}
        \centering
        \includegraphics[width=\linewidth]{Figures/cognitive_complexity_haystack.png}
    \end{subfigure}%
    \hfill
    \begin{subfigure}{0.33\textwidth}
        \centering
        \includegraphics[width=\linewidth]{Figures/cognitive_complexity_moto.png}
    \end{subfigure}
    
    % --- VERTICAL SPACING CONTROL ---
    \par\vspace{0.1cm} 
    
    % --- ROW 2 ---
    \begin{subfigure}{0.33\textwidth}
        \centering
        \includegraphics[width=\linewidth]{Figures/sqale_index_conan.png}
    \end{subfigure}%
    \hfill
    \begin{subfigure}{0.33\textwidth}
        \centering
        \includegraphics[width=\linewidth]{Figures/sqale_index_haystack.png}
    \end{subfigure}%
    \hfill
    \begin{subfigure}{0.33\textwidth}
        \centering
        \includegraphics[width=\linewidth]{Figures/sqale_index_moto.png}
    \end{subfigure}
    
\end{figure*}

==> Figures/figure_task_and_category_distribution.tex <==
\begin{figure*}[htbp]
    \centering
    
    % First row
    \begin{minipage}{\textwidth}
        \centering
        \begin{subfigure}[b]{0.3\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/repo_task_lists_pie.png}
            \caption{Standard}
            \label{fig:repo_task_pie}
        \end{subfigure}
        \hfill
        \begin{subfigure}[b]{0.3\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/repo_task_lists_pie_lite.png}
            \caption{Lite}
            \label{fig:repo_task_pie_lite}
        \end{subfigure}
        \hfill
        \begin{subfigure}[b]{0.3\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/repo_task_lists_pie_mini.png}
            \caption{Mini}
            \label{fig:repo_task_pie_mini}
        \end{subfigure}
        \caption{Repository task lists distribution (pie charts)}
        \label{fig:repo_task_lists}
    \end{minipage}
    
    \vspace{1em}
    
    % Second row
    \begin{minipage}{\textwidth}
        \centering
        \begin{subfigure}[b]{0.3\textwidth}
            \centering
            \includegraphics[width=\textwidth, height=0.18\textheight]{Figures/task_distribution_bar.png}
            \caption{Standard}
            \label{fig:task_dist_bar}
        \end{subfigure}
        \hfill
        \begin{subfigure}[b]{0.3\textwidth}
            \centering
            \includegraphics[width=\textwidth, height=0.18\textheight]{Figures/task_distribution_bar_lite.png}
            \caption{Lite}
            \label{fig:task_dist_bar_lite}
        \end{subfigure}
        \hfill
        \begin{subfigure}[b]{0.3\textwidth}
            \centering
            \includegraphics[width=\textwidth, height=0.18\textheight]{Figures/task_distribution_bar_mini.png}
            \caption{Mini}
            \label{fig:task_dist_bar_mini}
        \end{subfigure}
        \caption{Task distribution (bar charts)}
        \label{fig:task_distribution}
    \end{minipage}
    
\end{figure*}
